Two bijections on Tamari intervals

We use a recently introduced combinatorial object, the interval-poset, to describe two bijections on intervals of the Tamari lattice. Both bijections give a combinatorial proof of some previously known results. The first one is an inner bijection between Tamari intervals that exchanges the initial rise and lower contacts statistics. Those were introduced by Bousquet-M\'elou, Fusy, and Pr\'eville-Ratelle who proved they were symmetrically distributed but had no combinatorial explanation. The second bijection sends a Tamari interval to a closed flow of an ordered forest. These combinatorial objects were studied by Chapoton in the context of the Pre-Lie operad and the connection with the Tamari order was still unclear.

==> figures/interval-posets/I3-1.tex <==

% 1
% 2
% 3

\begin{tikzpicture}\node(T1) at (0,0) {1};\node(T2) at (0,-1) {2};\node(T3) at (0,-2) {3};\end{tikzpicture}

==> figures/interval-posets/I3-10.tex <==

%      1
% |    |
% 2 -- 3

\begin{tikzpicture}\node(T2) at (0,-1) {2};\node(T1) at (1,0) {1};\node(T3) at (1,-1) {3};\draw[color=blue] (T2) -- (T3);\draw[color=red] (T2) -- (T1);\draw[color=red] (T3) -- (T1);\end{tikzpicture}



==> figures/interval-posets/I3-11.tex <==

% 1
% 2
% |
% 3

\begin{tikzpicture}\node(T1) at (0,0) {1};\node(T2) at (0,-1) {2};\node(T3) at (0,-2) {3};\draw[color=red] (T3) -- (T2);\end{tikzpicture}



==> figures/interval-posets/I3-13.tex <==

% 1
% |
% 2
% |
% 3

\begin{tikzpicture}\node(T1) at (0,0) {1};\node(T2) at (0,-1) {2};\node(T3) at (0,-2) {3};\draw[color=red] (T2) -- (T1);\draw[color=red] (T3) -- (T2);\end{tikzpicture}




==> figures/interval-posets/I3-2.tex <==

% 1 -- 2
% 3

\begin{tikzpicture}\node(T1) at (0,0) {1};\node(T2) at (1,0) {2};\node(T3) at (1,-1) {3};\draw[color=blue] (T1) -- (T2);\end{tikzpicture}

==> figures/interval-posets/I3-3.tex <==

% 1
% 2 -- 3

\begin{tikzpicture}\node(T1) at (0,0) {1};\node(T2) at (0,-1) {2};\node(T3) at (1,-1) {3};\draw[color=blue] (T2) -- (T3);\end{tikzpicture}

==> figures/interval-posets/I3-4.tex <==

% 1 -- 3
% 2 -- 

\begin{tikzpicture}\node(T1) at (0,0) {1};\node(T2) at (0,-1) {2};\node(T3) at (1,0) {3};\draw[color=blue] (T1) -- (T3);\draw[color=blue] (T2) -- (T3);\end{tikzpicture}

==> figures/interval-posets/I3-5.tex <==

% 1 -- 2 -- 3

\begin{tikzpicture}\node(T1) at (0,0) {1};\node(T2) at (1,0) {2};\node(T3) at (2,0) {3};\draw[color=blue] (T1) -- (T2);\draw[color=blue] (T2) -- (T3);\end{tikzpicture}

==> figures/interval-posets/I3-6.tex <==

% 1
% |
% 2
% 3

\begin{tikzpicture}\node(T2) at (0,-1) {2};\node(T1) at (0,0) {1};\node(T3) at (0,-2) {3};\draw[color=red] (T2) -- (T1);\end{tikzpicture}


==> figures/interval-posets/I3-7.tex <==

% 1
% |
% 2 -- 3

\begin{tikzpicture}\node(T2) at (0,-1) {2};\node(T1) at (0,0) {1};\node(T3) at (1,-1) {3};\draw[color=blue] (T2) -- (T3);\draw[color=red] (T2) -- (T1);\end{tikzpicture}



==> figures/interval-posets/I3-8.tex <==

% 1 -- 3
% |
% 2 -- 

\begin{tikzpicture}\node(T2) at (0,-1) {2};\node(T1) at (0,0) {1};\node(T3) at (1,0) {3};\draw[color=blue] (T1) -- (T3);\draw[color=blue] (T2) -- (T3);\draw[color=red] (T2) -- (T1);\end{tikzpicture}



==> figures/interval-posets/I3-9.tex <==

%      1
% |    |
% 2    3

\begin{tikzpicture}\node(T2) at (0,-1) {2};\node(T1) at (1,0) {1};\node(T3) at (1,-1) {3};\draw[color=red] (T2) -- (T1);\draw[color=red] (T3) -- (T1);\end{tikzpicture}



==> figures/interval-posets/I5-ex1.tex <==

% 1
% 
% 2 
%       
% 3 -- 4
%      |
%      5


\begin{tikzpicture}\node(T1) at (0,0) {1};\node(T2) at (0,-1) {2};\node(T3) at (0,-2) {3};\node(T4) at (1,-2) {4};\node(T5) at (1,-3) {5};\draw[color=blue] (T3) -- (T4);\draw[color=red] (T5) -- (T4);\end{tikzpicture}



==> figures/interval-posets/I5-ex2.tex <==

% 1
% |
% 2 
%       
% 3 -- 4
%      |
%      5


\begin{tikzpicture}\node(T2) at (0,-1) {2};\node(T1) at (0,0) {1};\node(T3) at (0,-2) {3};\node(T4) at (1,-2) {4};\node(T5) at (1,-3) {5};\draw[color=red] (T2) -- (T1);\draw[color=blue] (T3) -- (T4);\draw[color=red] (T5) -- (T4);\end{tikzpicture}



==> figures/interval-posets/I5-ex3.tex <==

%      1
% |    |
% 2    3 -- 4
%           |
%           5


\begin{tikzpicture}\node(T2) at (0,-1) {2};\node(T3) at (1,-1) {3};\node(T1) at (1,0) {1};\node(T4) at (2,-1) {4};\node(T5) at (2,-2) {5};\draw[color=red] (T2) -- (T1);\draw[color=blue] (T3) -- (T4);\draw[color=red] (T3) -- (T1);\draw[color=red] (T5) -- (T4);\end{tikzpicture}




==> figures/interval-posets/I5-ex4.tex <==

%           1
% |    |    |
% 2    3 -- 4
%           |
%           5


\begin{tikzpicture}\node(T2) at (0,-1) {2};\node(T3) at (1,-1) {3};\node(T1) at (2,0) {1};\node(T4) at (2,-1) {4};\node(T5) at (2,-2) {5};\draw[color=red] (T2) -- (T1);\draw[color=blue] (T3) -- (T4);\draw[color=red] (T3) -- (T1);\draw[color=red] (T4) -- (T1);\draw[color=red] (T5) -- (T4);\end{tikzpicture}




==> figures/interval-posets/big-ex--10.tex <==
\begin{tikzpicture}
  \node(T1) at (0,0) {1};
  \node(T2) at (1,0) {2};

  \draw[color=blue] (T1) -- (T2);
\end{tikzpicture}


==> figures/interval-posets/big-ex--7.tex <==
\begin{tikzpicture}
  \node(T2) at (0,-1) {2};
  \node(T1) at (1,0) {1};
  \node(T3) at (1,-1) {3};

  \draw[color=blue] (T2) -- (T3);
  \draw[color=red] (T2) -- (T1);
  \draw[color=red] (T3) -- (T1);
\end{tikzpicture}


==> figures/interval-posets/big-ex--9.tex <==
\begin{tikzpicture}
  \node(T1) at (0,0) {1};
\end{tikzpicture}


==> figures/interval-posets/big-ex-3.tex <==
\begin{equation}
  \beta(I_{1}) =
  \scalebox{0.5}{\input{figures/interval-posets/big-ex--7}},
\end{equation}


==> figures/interval-posets/big-ex-5.tex <==
\begin{equation}
  \beta(I_{2}) =
  \scalebox{0.5}{\input{figures/interval-posets/big-ex--10}},
\end{equation}


==> figures/interval-posets/big-ex.tex <==
\begin{equation}
\scalebox{0.5}{\input{figures/interval-posets/big-ex--1}} \leftrightarrow
\left( \scalebox{0.5}{\input{figures/interval-posets/big-ex--2}},
\scalebox{0.5}{\input{figures/interval-posets/big-ex--3}},
2 \right)
\end{equation}


==> figures/trees/T3-1-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T3-1.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.750, -0.500){};
\node (N000) at (0.250, -1.000){};
\draw[Point] (N000) circle;
\draw (N00.center) -- (N000.center);
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T3-2-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T3-2.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.250, -0.500){};
\node (N001) at (0.750, -1.000){};
\draw[Point] (N001) circle;
\draw (N00.center) -- (N001.center);
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T3-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T3-3.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (1.250, -0.500){};
\node (N010) at (0.750, -1.000){};
\draw[Point] (N010) circle;
\draw (N01.center) -- (N010.center);
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T3-4-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T3-4.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}
\node (N0) at (0.750, 0.000){};
\node (N00) at (0.250, -0.500){};
\draw[Point] (N00) circle;
\node (N01) at (1.250, -0.500){};
\draw[Point] (N01) circle;
\draw (N0.center) -- (N00.center);
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T3-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T3-5.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (0.750, -0.500){};
\node (N011) at (1.250, -1.000){};
\draw[Point] (N011) circle;
\draw (N01.center) -- (N011.center);
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T4-1-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%      /
%     /
%    /

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (1.500, -2.000){2};
\node (N0000) at (0.500, -3.000){1};
\draw (N000) -- (N0000);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-10-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%      ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\node (N0100) at (1.500, -3.000){2};
\draw (N010) -- (N0100);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-11-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%         \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (1.500, -2.000){2};
\node (N0101) at (2.500, -3.000){3};
\draw (N010) -- (N0101);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-12-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%         \.
%        ./ \.
%        

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N010);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-14-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%         \.
%           \.
%             \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\node (N0111) at (3.500, -3.000){4};
\draw (N011) -- (N0111);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-2-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./
%     \

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (0.500, -2.000){1};
\node (N0001) at (1.500, -3.000){2};
\draw (N000) -- (N0001);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./\.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\node (N001) at (2.500, -2.000){3};
\draw (N00) -- (N000);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%      ./
%       \.
%        \.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\node (N0011) at (2.500, -3.000){3};
\draw (N001) -- (N0011);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-6-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%     ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\node (N01) at (3.500, -1.000){4};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-7-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%       \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\node (N01) at (3.500, -1.000){4};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-8-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%        ./

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\draw (N01) -- (N010);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-9-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%           \.

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N011);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}
